Using PPP Information to Implement a Global Real-Time Virtual Network DGNSS Approach

Differential GNSS (DGNSS) has been demonstrated to provide reliable, high-quality range correction information enabling real-time navigation with centimeter to sub-meter accuracy, which is required for applications such as connected and autonomous vehicles. However, DGNSS requires a local reference station near each user. For a continental or global scale implementation, this information dissemination approach would require a dense network of reference stations whose construction and maintenance would be prohibitively expensive. Precise Point Positioning affords more flexibility as a public service for GNSS receivers, but its State Space Representation format is not supported by most receivers in the field or on the market. This article proposes a novel Virtual Network DGNSS (VN-DGNSS) approach and an optimization algorithm that is key to its implementation. The approach capitalizes on the existing PPP infrastructure without the need for new physical reference stations. By connecting to public GNSS SSR data services, a VN-DGNSS server maintains current information about common-mode errors. Construction of the RTCM Observation Space Representation messages from this SSR information requires both the signal time-of-transmission and the satellite position at that time which are consistent with the time-of-reception for each client. This article presents an algorithm to determine these quantities. The results of real-time stationary and moving platform evaluations are included, using u-blox M8P and ZED-F9P receivers. The performance surpasses the SAE specification (68% of horizontal error <= 1.5 m and vertical error <= 3 m) and shows significantly better horizontal performance than GNSS Open Service. The moving tests also show better horizontal performance than the ZED-F9P receiver with SBAS enabled and achieve the lane-level accuracy (95% of horizontal errors less than 1 meter).

==> sections/apdB.tex <==
\clearpage
\red
\subsection{Satellite position estimation (rover respective)}
Let's review the common process to calculate satellite position. The user will have the pseudorange measurements $\tilde{\rho}^s_{f,r}(t_r)$ and receiver time $t_r$. To simplify the description and consistent with the Eqn. (\ref{eqn:RTCM}), assuming this receiver do not have clock bias. Revise the Eqn. (\ref{eqn:codeM}) by
	\begin{equation}\label{eqn:apb}
	\left.
	\begin{aligned}
		\tilde{\rho}^s_{f,r} (t_r) = &R\Big(\BoldP_r(t_r), \hat{\BoldP}^s(t^s)\Big) + E_r^s(t^s) 
		- c \, \Delta dt^s 
		+ c \, B_f^s \\
		&+ T^s_r + I^s_{f,r} + M^s_{f,r} + \eta^s_{f,r},
	\end{aligned}
	\right\}
	\end{equation}

The propagation pseudo-time $t^{'}_p = \tilde{\rho}^s_{f,r}/c$. Hence we can get signal transmit pseudo-time $\hat{t}^s = t_r - t^{'}_p$ (To matching Jay's book Appendix C, The $\hat{t}^s$ is identical to $t_{sv}$ in the book). As what mentioned before, $[\hat{\BoldP}^s(t^s),\hat{\BoldV}^s(t^s),\hat{dt}^s(t^s)] = f(\hat{t}^s,\Boldtheta_e^s)$. 

The transmit time $t = \hat{t}^s + \Delta dt^s - B_f^s$ (similar to $t = t_{sv}-\Delta t_{sv}$ in the book, but the book ignored the satellite hardware bias $B_f^s$).

Let's think about one aspect, define
\begin{equation}
	t^{'}_p = t^d_p - \Delta dt^s + B_f^s + e^s_r,
\end{equation}
where $t^d_p = \frac{R\Big(\BoldP_r(t_r), \hat{\BoldP}^s(t^s)\Big)}{c}$ as position direct travel time, $e^s_r = \frac{E_r^s(t^s) + T^s_r + I^s_{f,r} + M^s_{f,r} + \eta^s_{f,r}}{c}$ as time delay caused by errors, and $\Delta dt^s = \hat{dt}^s(t^s) + \delta dt^s$ where $\delta dt^s$ is the residual satellite clock error. (Not officially technical, but to get the basic idea below.)

The magnitude of total error $t_{err} = -\delta dt^s + B_f^s + e^s_r$ is less than 200 ns. Then,
\begin{equation}
	t^{'}_p = t^d_p - \hat{dt}^s(t^s) + t_{err},
\end{equation}
 Considering the satellite moving speed is about 4000 m/s, if $t_{err}$ is magically removed from $t^{'}_p$, would the satellite position calculation $\hat{\BoldP}^s(t^s)$ be significantly affected? The answer obviously is not.
Hence, assuming we have the error-free propagation pseudo-time $t^e_p = t^{'}_p - t_{err}$ (actually $t_{err}$ is unknown), the new signal transmit pseudo-time will be 
\begin{equation}
\hat{t}^s_{new} = t_r - t^e_p. 
\end{equation}
The difference between $f(\hat{t}^s,\Boldtheta_e^s)$ and $f(\hat{t}^s_{new},\Boldtheta_e^s)$ are negligible. We will still get almost the same (difference for satellite position $\Delta \BoldP^s$ less than 0.008m) $\hat{\BoldP}^s,\hat{\BoldV}^s$, and $\hat{dt}^s$ whatever $t_{err}$ exist or not. For the range, note that by Taylor series,
\begin{equation}
	R\Big(\BoldP_b, \hat{\BoldP}^s({t}^s)+\Delta \BoldP^s\Big) 
	= R\Big(\BoldP_b,  \hat{\BoldP}^s({t}^s)\Big)
	+ \left(\1_b^s \,\cdot\, \BoldV^s \right) \, \Delta \BoldP^s.
\end{equation}
and $\1_b^s\cdot\BoldV^s$ is even smaller.

Getting confused? Let's state it by a different way. In mathematical computation process, we have pseudorange No.1 $\tilde{\rho}^s_{1}$ from Eqn. (\ref{eqn:apb}) and No.2 $\tilde{\rho}^s_{2} = R\Big(\BoldP_r(t_r), \hat{\BoldP}^s(t^s)\Big) - c \,\hat{dt}^s$ under the condition of the same $t_r$. The differences in the results of $f(\hat{t}^s,\Boldtheta_e^s)$ are negligible.

The above discussion is for calculating the satellite position. Then, let's go the objective. If we know $\BoldP_r(t_r)$ and $t_r$, how to estimate $\hat{\BoldP}^s(t^s)$? Based on the discussion in the last paragraph, it's feasible to estimate it even we don't know the value of error terms. 
\begin{itemize}
	\item 1. Given an reasonable initial value for the error-ignored propagation pseudo-time $t_p$. Here the model for $c\times t_p = R(\BoldP_b,\hat{\BoldP}^s(t^s)) - c \,\hat{dt}^s$.
	\item 2. Given an initial for-loop previous value $t_p^{-} = 0$.
	\item 3. If $|t^-_p - t_p|>10^{-11}$, do following, otherwise jump to step...
	\item 4. Signal transmit pseudo-time $\hat{t}^s = t_r - t_p$.
	\item 5. $[\hat{\BoldP}^s(t^s),\hat{\BoldV}^s(t^s),\hat{dt}^s(t^s)] = f(\hat{t}^s,\Boldtheta_e^s)$ for getting the satellite position, velocity and clock bias correction.
	\item 6. Range by position: $R_1 = R(\BoldP_b,\hat{\BoldP}^s(t^s))$
	\item 7. Range by travel time: $R_2 = c~(t_p+\hat{dt}^s(t^s))$ (Based on the model at step 1).
	\item 8. The goal is to achieve $F = R_1 - R_2$ to zero.
	\item 9. $dF = -\frac{\hat{\BoldV}^s(t^s)\cdot (\hat{\BoldP}^s-\BoldP_b)}{R_1}-c\,\left(1 - \frac{\partial}{\partial t_p}\hat{dt}^s(\hat{t}^s)\right)$
	\item 10. Save the previous value: $t_p^{-} = t_p$.
	\item 11. By Newton's Zero Finding Algorithm: $t_p = t_p - \frac{F}{dF}$.
	\item 12. Back to step 3.
	\item 13. Signal transmit time $t_s = t_r - t_p + \hat{dt}^s(t^s)$.
	\item 14. Output $\hat{\BoldP}^s(t^s)$ and $\hat{dt}^s(t^s)$ for compute the Eqn. (\ref{eqn:RTCM}). Output $t_s$ for using the SSR clock product. Comparing to the reality, $t_r - t_p + \hat{dt}^s(t^s)$ does not account for $t_{err}$. But the effect of $t_{err}$ (less than 200 ns) is negligible for clock correction Eqn. (\ref{eqn:clkcorr}).
\end{itemize}




==> sections/apdC.tex <==
\clearpage
\subsection{Revised version of satellite position estimation (server respective)}
\blue
{\red Pursuing the discussion in Appendix B but independent to B.}
To enable computation of the first line of eqn. (\ref{eqn:RTCM}),
the goal of this section is to determine the satellite position
$\hat{\BoldP}^s(t^s)$ for a signal received from satellite $s$ at time $t_b$.  
This requires computation of both  the satellite transmit time $t^s$ and the satellite position at the at time $\hat{\BoldP}^s(t^s)$.


The ICD provides equations to compute the satellite position $\hat{\BoldP}^s (t^s)$ and satellite clock offset $\hat{dt}^s$.
These equations use data in the broadcast navigation message.
%
In a user respective, the base station transmit its RAW measurements to user. The computation would depend on the signal pseudo-transmit-time $\hat{t}^s$ that would be calculated by $\hat{t}^s = t_b - \tilde{\rho}^s_{f,b}/c$ where $\tilde{\rho}^s_{f,b}$ is the code (pseudorange) measurement from base station. Let $t^{'}_p = \tilde{\rho}^s_{f,b}/c$ denotes the propagation pseudo-time.
In VN-DGNSS approach, $\hat{\BoldP}^s (t^s)$ must be estimated by optimizing the propagation pseudo-time $t^{'}_p$.

Re-define
\begin{equation}\label{eqn:tp_prime}
	t^{'}_p = t^d_p - \hat{dt}^s(t^s) + t_{err},
\end{equation}
where $t^d_p = \frac{R\Big(\BoldP_r(t_r), \hat{\BoldP}^s(t^s)\Big)}{c}$ as range direct travel time, $t_{err} = -\delta dt^s + B_f^s + e^s_b$ denotes both common-mode and non-common-mode errors scaled to units of time (i.e., $|t_{err}|\le 200$ ns) where $e^s_r = \frac{E_r^s(t^s) + T^s_r + I^s_{f,r} + M^s_{f,r} + \eta^s_{f,r}}{c}$, and $\Delta dt^s = \hat{dt}^s(t^s) + \delta t^s$ ({\red The section II need define $\Delta dt^s$}).

If $t_{err}$ is removed from $t^{'}_p$, assuming the error-free propagation pseudo-time $t_p = t^{'}_p - t_{err}$ (actually $t_{err}$ is unknown), the new signal transmit pseudo-time will be 
\begin{equation}
	\hat{t}^s_{new} = t_r - t_p. 
\end{equation}
The difference between $f(\hat{t}^s,\Boldtheta_e^s)$ and $f(\hat{t}^s_{new},\Boldtheta_e^s)$ are $[\Delta \hat{\BoldP}^s,\Delta \hat{\BoldV}^s,\Delta \hat{dt}^s]$. Because the satellite moving speed is about 4000 m/s, the magnitude of $\Delta \BoldP^s$ less than 0.008m. The effects $\Delta \hat{\BoldV}^s$ and $\Delta \hat{dt}^s$ are negligible. For the range, note that by Taylor series,
\begin{equation}
	R\Big(\BoldP_b, \hat{\BoldP}^s({t}^s)+\Delta \BoldP^s\Big) 
	= R\Big(\BoldP_b,  \hat{\BoldP}^s({t}^s)\Big)
	+ \left(\1_b^s \,\cdot\, \BoldV^s \right) \, \Delta \BoldP^s.
\end{equation}
and $\1_b^s\cdot\BoldV^s$ is even smaller. Therefore, the effects of $\Delta \BoldP^s$ are negligible to the satellite range computation.

To estimate the satellite position without real measurements, the objective is to optimize the error-free propagation pseudo-time $t_p$. Algorithm \ref{alg:svpos} computes the satellite position $\hat{\BoldP}^s(t^s)$ by minimizing the square of the error between the two range equations:
\begin{align}\label{eqn:F_defn}
	F(t_p: \BoldP_b, \, {t}_b) 
	&= \left(R\Big(\BoldP_b, \hat{\BoldP}^s(t^s)\Big) 
	- c \, t^d_p\right)
\end{align}
as a function of the propagation time $t_p$ where $t^d_p$ is computed by $t^d_p = t_p+\hat{dt}^s(t^s)$ related to Eqn. (\ref{eqn:tp_prime}).
The notation $	F(t_p: \, \BoldP_b, \, {t}_b) $ means that $t_p$ is the argument and $\BoldP_b$ and ${t}_b$ are known parameters.
For the numeric search, the propagation time is initialized to $t_p = 0.067$ seconds because GNSS satellites are approximately 20,000 km from the Earth surface.
Step \ref{alg1:t^s} computes the pseudo-transmit time $\hat{t}^s$, 
which is used in Step \ref{alg1:eph} to compute the
broadcast 
clock correction $\hat{dt}^s(\hat{t}^s)$,
satellite position $\hat{\BoldP}^s(t^s)$,  and 
velocity $\hat{V}^s(t^s)$.
The ICD models \cite{icd2013global,galileo2008galileo,beidou2012beidou} are represented by the function $f(\hat{t}^s,\Boldtheta_e^s)$ where $\Boldtheta_e^s$ are the ephemeris parameters, provided to the server by internet source, for example, the BKG data streams.
Steps \ref{alg1:r1} - \ref{alg1:F} compute the two ranges and the range error for the current value of $t_p$.
Step \ref{alg1:partial} computes the partial derivative
\begin{align}\nonumber
	\frac{\partial F}{\partial t^s_p}&=\frac{\partial }{\partial \hat{\BoldP}^s} 
	R\Big(\BoldP_b, \hat{\BoldP}^s\Big)%|_{\hat{\BoldP}^s=\hat{\BoldP}^s(t^s)}
	%
	\frac{\partial \hat{\BoldP}^s}{\partial \bar{t}^s} 
	%
	\frac{\partial  \bar{t}^s}{\partial \hat{t}^s}
	%
	\frac{\partial  \hat{t}^s}{\partial t^s_p}   - c \,\frac{\partial}{\partial t^s_p}(t^s_p + \hat{dt}^s(\hat{t}^s)) \\
	&= -\left(\1_b^s \cdot \hat{\BoldV}^s\right)
	%
	\left( 1 - a_1 - 2\, a_2 \, (\hat{t}^s-toc)\right) - c - c\,\frac{\partial \hat{dt}^s(\hat{t}^s)}{\partial \hat{t}^s}\frac{\partial \hat{t}^s}{\partial t^s_p} \\
	&= -\left(\1_b^s \cdot \hat{\BoldV}^s\right)
	%
	\left( 1 - a_1 - 2\, a_2 \, (\hat{t}^s-toc)\right)\label{eqn:partial1} - c + c\,\Big(a_1+2\,a_2 (\hat{t}_s-toc)\Big)
\end{align}
where $\1_b^s = \frac{(\hat{\BoldP}^s-\BoldP_b)}{R_1}$, $a_i$ and $toc$ are the parameters of the satellite clock correction model as defined in the ICD. It's needed to mention that the magnitude of $a_1$ is $10^{-11}$ and $a_2$ is even smaller.

Step \ref{alg1:Newton} implements Newton's Zero Finding Algorithm proceed below is to optimize the propagation time $t_p = t_b - \hat{t}^s$ to minimize the quare of the error defined in eqn. (\ref{eqn:F_defn}).
The resulting output provides the satellite location $\hat{\BoldP}^s(t^s)$ which enables computation of 
$R\Big(\BoldP_b, \hat{\BoldP}^s(t^s)\Big)$ and satellite clock correction $\hat{dt}^s$ 
as required for the RTCM OSR measurement defined in eqn. (\ref{eqn:RTCM}). The output signal transmit time $t_s$ is used in the SSR clock product.




%	\begin{minipage}[tbh]{\linewidth}
\begin{algorithm}[b]
	\caption{Satellite Position Estimation}      
	\label{alg:svpos}               
	\begin{algorithmic}[1]
		\Require $\BoldP_b$, $t_b$.
		\Ensure $\hat{\BoldP}^s(t^s)$, $\hat{V}^s(t^s)$, $\hat{dt}^s$ and $t^s$.
		\State $t_p = 0.067$; {\color{lgray}// Initialize the propagation time $t_p$}
		\State $t^-_p = 0$;  
		\While{$|t^-_p - t_p|>10^{-11}$}
		\State $\hat{t}^s = t_b - t_p$; 
		{\color{lgray}// Pseudo-transmit time} 
		\label{alg1:t^s}
		\State $[\hat{\BoldP}^s(t^s),\hat{\BoldV}^s(t^s),\hat{dt}^s(\hat{t}^s)] = f(\hat{t}^s,\Boldtheta_e^s)$;  {\color{lgray}// ICD models}
		\label{alg1:eph}
		\State $R_1 = R(\BoldP_b,\hat{\BoldP}^s(t^s))$ 
		{\color{lgray}// Range computed based on position}
		\label{alg1:r1}
		\State $t^d_p = t_p + \hat{dt}^s(\hat{t}^s)$ {\color{lgray}// See definition in eqn. (\ref{eqn:F_defn})}
		\State $R_2 =c \cdot t^d_p  $ {\color{lgray}// Range computed based on propagation time}
		\State $F = R_1 - R_2$;	
		{\color{lgray}// Eqn. (\ref{eqn:F_defn}) }
		\label{alg1:F}
		\State $dF = \frac{\partial F}{\partial \hat{t}^s}\frac{\partial \hat{t}^s}{\partial t_p} - c \,\frac{\partial}{\partial t_p}(t_p + \hat{dt}^s(\hat{t}^s))$;
		{\color{lgray}// Eqn. (\ref{eqn:partial1})}
		\label{alg1:partial} 
		\State $t^-_p = t_p$; {\color{lgray}// save the previous value}
		\State $t_p = t_p - \frac{F}{dF}$; {\color{lgray}// Newton's Zero Finding Algorithm}\label{alg1:Newton} 
		\EndWhile
		\State $t^s = t_r - t_p + \hat{dt}^s(\hat{t}^s)$. {\color{lgray}// Signal transmit time}
	\end{algorithmic}
\end{algorithm}
%	\end{minipage}

